The Power of Both Choices: Practical Load Balancing for Distributed Stream Processing Engines

We study the problem of load balancing in distributed stream processing engines, which is exacerbated in the presence of skew. We introduce Partial Key Grouping (PKG), a new stream partitioning scheme that adapts the classical "power of two choices" to a distributed streaming setting by leveraging two novel techniques: key splitting and local load estimation. In so doing, it achieves better load balancing than key grouping while being more scalable than shuffle grouping. We test PKG on several large datasets, both real-world and synthetic. Compared to standard hashing, PKG reduces the load imbalance by up to several orders of magnitude, and often achieves nearly-perfect load balance. This result translates into an improvement of up to 60% in throughput and up to 45% in latency when deployed on a real Storm cluster.

==> sections/notes.tex <==
%
\section{Notes}
\begin{enumerate}
\item Load balancing in streams is an important issue when input distribution of keys is skewed
\begin{enumerate}
\item Current solutions do not work for different reasons (key grouping, shuffle grouping)
\item Hasn’t been studied well so far
\item Setting is Storm-like (no key identity in PE, no key migration possible)
\end{enumerate}
\item We propose to use PoTC to address the issue (nothing new here)
\begin{enumerate}
\item PoTC with “sticky” key grouping would give already good results (David’s simulations + proofs)
\item However PoTC can’t be used out of the box with multiple sources because there is a coordination problem (need to remember and have consensus on which of the choices is taken)
\end{enumerate}
\item We propose partial key grouping (``key splitting'') to address this issue (needs additional merge phase like shuffle grouping)
\begin{enumerate}
\item This requires a slightly different programming paradigm, which however has many applications (word count, naive bayes, sketches, SPDT)
\item We show that it works even better than normal PoTC (proof? and simulations)
\item Does not require coordination among sources (but requires load estimation)
\end{enumerate}
\item We propose local load estimation at the sources in a practical scenario
\begin{enumerate}
\item Compare with omniscient oracle (simulations)
\item Assess if some lightweight form of communication with destinations is useful (?) (simulations?)
\end{enumerate}
\item If the number of destinations/bins B are too many the load is unbalanced anyway
\begin{enumerate}
\item Key splitting helps in this case (explore power of d choices for $d>2$)
\end{enumerate}
\item We modify Storm to implement partial key grouping
\begin{enumerate}
\item Tests on live system
\item Release code
\end{enumerate}
\end{enumerate}

\section{Naming Conventions}

\begin{table}[htdp]
\caption{default}
\begin{center}
\begin{tabular}{l p{0.7\columnwidth}}
Partition		&	a division of the stream into sub-streams \\
Grouping		&	see Partition \\
Sub-Stream	&	a portion of the stream created by a partition \\
Message		&	an element of a stream, composed by a Key-Value pair \\
Tuple		&	see Message \\
Key			&	part of a Message that represents its identity \\
Stream		&	an infinite sequence of keyed messages \\
Key splitting	&	assigning a key to multiple (2) \peis \\
Power of both choices	&	see Key splitting \\
Static \potc	&	power of two choices \emph{without} key splitting \\
\end{tabular}
\end{center}
\label{default}
\end{table}%

